Insights from the Frontline: GenAI Utilization Among Software Engineering Students

Generative AI (genAI) tools (e.g., ChatGPT, Copilot) have become ubiquitous in software engineering (SE). As SE educators, it behooves us to understand the consequences of genAI usage among SE students and to create a holistic view of where these tools can be successfully used. Through 16 reflective interviews with SE students, we explored their academic experiences of using genAI tools to complement SE learning and implementations. We uncover the contexts where these tools are helpful and where they pose challenges, along with examining why these challenges arise and how they impact students. We validated our findings through member checking and triangulation with instructors. Our findings provide practical considerations of where and why genAI should (not) be used in the context of supporting SE students.

==> _tex_folder/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> _tex_folder/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> sec/TODO.tex <==
Vocab check:
- Students' possessive, Participants' possessive - done
- Script and not guide - done


% References to add:
% @article{kim2024chatgpt,
%   title={ChatGPT in Data Visualization Education: A Student Perspective},
%   author={Kim, Nam Wook and Ko, Hyung-Kwon and Myers, Grace and Bach, Benjamin},
%   journal={arXiv preprint arXiv:2405.00748},
%   year={2024}
% }
% This work explores the impact of ChatGPT on student
% learning in a data visualization course. Throughout the semester, students engaged with ChatGPT across four distinct projects, designing and implementing data visualizations using a variety of tools such as
% Tableau, D3, and Vega-lite. Collected conversation logs and
% reflection surveys after each assignment and conducted interviews
% with selected students to gain deeper insights into their experiences with ChatGPT. analysis examined the advantages
% and barriers of using ChatGPT, students’ querying behavior,
% the types of assistance sought, and its impact on assignment
% outcomes and engagement. 

% @inproceedings{padiyath2024insights,
%   title={Insights from Social Shaping Theory: The Appropriation of Large Language Models in an Undergraduate Programming Course},
%   author={Padiyath, Aadarsh and Hou, Xinying and Pang, Amy and Viramontes Vargas, Diego and Gu, Xingjian and Nelson-Fromm, Tamara and Wu, Zihan and Guzdial, Mark and Ericson, Barbara},
%   booktitle={Proceedings of the 2024 ACM Conference on International Computing Education Research-Volume 1},
%   pages={114--130},
%   year={2024}
% } 
% Through a series of learning performance, surveys, and interviews, they found that students internalize technological determinism narratives, and that these were shaped by peer use and perceptions of future jobs requiring use of LLMs. But students were very self-aware of the negative impacts on their learning and changed their behavior, demonstrating that how LLMs are used are very much socially shaped, not technology determined.

% INCLUDED
% @inproceedings{prather2024widening,
%   title={The Widening Gap: The Benefits and Harms of Generative AI for Novice Programmers},
%   author={Prather, James and Reeves, Brent N and Leinonen, Juho and MacNeil, Stephen and Randrianasolo, Arisoa S and Becker, Brett A and Kimmel, Bailey and Wright, Jared and Briggs, Ben},
%   booktitle={Proceedings of the 2024 ACM Conference on International Computing Education Research-Volume 1},
%   pages={469--486},
%   year={2024}
% }
% Through participant observation, eye tracking, and interviews (replicating a prior study on metacognition), they found that when students used Github Copilot, students with no metacognitive difficulties were able to use Copilot to accelerate their problem solving; the students that did have metacognitive difficulties exacerbated metacognitive difficulties and encountered new ones, amplifying disparities in learning outcomes and harming self-efficacy. 

% INCLUDED
% @inproceedings{skripchuk2024investigation,
%   title={An Investigation of the Drivers of Novice Programmers' Intentions to Use Web Search and GenAI},
%   author={Skripchuk, James and Bacher, John and Price, Thomas},
%   booktitle={Proceedings of the 2024 ACM Conference on International Computing Education Research-Volume 1},
%   pages={487--501},
%   year={2024}
% }
% investigated students intentions around using web resources and generative AI. He argued that LLMs are not so different from use of web resources, and investigate students’ choices around whether to use web or generative AI resources. Through a scenario-based survey, they found that students generally assess the utility of resources, while accounting for plagiarism policing around use, but also peer opinions about resource use



==> sec/intro-copy.tex <==
\section{Introduction}
\label{sec:intro}

** GAI is being used everywhere and SE is no exception

** Students in SE need personalized help
    - Lit shows chatbots can help
    - Lit also warns against using GAI for education.

** We wanted to see how SE students are using GAI/where they succeed or suffer?
-> RQs
-> Takeaway for Educators: where (not) to integrate. AI designers: what to improve

\textbf{What's the problem?}

Educators don't know where/when genAI embedding works.

\textbf{Why is it a problem?}
Students are using it ad hoc, taking away from learning/problem solving. Getting answers and understanding it is not the same as coming up with one. Problem solving skill is boiled down to reading comprehension.

\textbf{What did we do?}
	Investigated student experiences with genAI usage in SE Learning: 
Learning Concepts, Implementation
  
\textbf{So what?}
Clear cases where genAI fails 
talk about this in class
Keep in mind when using it/embedding it

From our data, genAI suits/helps students in <<Benefits>> but with these caveats.
Those who want to cheat/bypass learning we are not catering to them, rather we are looking for things to avoid for people who really want to learn if genAI is to be used as a learning resource.

RQs:

* What is the landscape of genAI use amongst SE students?
 - When do they use it? (moments)
 - Where and how do they use it?
 - What are their perceived benefits and challenges?
 

O/P: Where they use, how they use, Benefits, Challenges, (across 4 quadrants)

* What are the causes and consequences of the challenges faced by students?
- What are the similarities and differences in these associations for learning and implementations?

O/P: Faults - Challenges - Impact

Need to \textbf{emphasize} on novelty:

Our novelty is not in finding challenges, or faults, or benefits.

Our novelty lies in showing the landscape, where good, where not good.

Our novelty lies in showing the associations of why these challenges occur and how they lead to student impacts. 




\iffalse
### Throwaway Ideas - ambu
In contemporary educational settings, the integration of Artificial Intelligence (AI) tools has become increasingly prevalent, extending even into traditionally complex subjects such as Software Engineering (SE). Among these AI tools, Generative AI (GenAI) has emerged as a potential aid for enhancing student learning experiences. While existing literature suggests the promise of AI, particularly in providing personalized support through mechanisms like chatbots, cautionary perspectives highlight the need for a nuanced understanding of its application in education.

This research aims to delve into the practicalities of GenAI utilization among students engaged in learning Software Engineering. By examining both successes and challenges, we seek to understand the nuanced landscape of its integration. A central concern driving this inquiry is the lack of clarity among educators regarding optimal contexts for GenAI application in SE education. This lack of clarity overshadows critical pedagogical goals, particularly the cultivation of problem-solving skills among students.

To address this gap, our study delves into the lived experiences of students utilizing GenAI in SE learning environments. Through our investigation, we aim to provide actionable insights for educators, outlining contexts where GenAI proves beneficial and where it may fall short.

Furthermore, our approach emphasizes the importance of understanding nuances within student experiences. We aim not only to identify challenges and benefits but also to elucidate the underlying associations between these factors and their impact on student learning outcomes. In doing so, our study seeks to offer pragmatic guidance for educators and AI developers alike, fostering a more informed approach to integrating GenAI tools into SE education.



\fi

==> sec/leftover-text.tex <==
% Method

% We aligned our exploration with an educational framework, i.e., Bloom’s taxonomy \cite{krathwohl2002revision, forehand2005bloom}, to guide the interpretation of students’ experiences in using genAI tools during SE courses. Bloom's taxonomy organizes learning objectives along a continuum of cognitive processes: from lower-order processes, which include the acquisition and understanding of knowledge (remembering, understanding), to higher-order processes that promote the application and synthesis of knowledge in new contexts (applying, analyzing, evaluating, and creating). Within the context of engineering educational objectives and outcomes, these processes correspond to \textit{conceptual learning} and \textit{practical implementations} \cite{felder2003designing, ambrose2010learning}.
% 
% Learning is a continuum of processes: starting from acquisition and understanding of knowledge to application and synthesis of knowledge in new contexts [CITE]. Within the context of engineering education, these processes range from learning of SE concepts to practical implementations [CITE]. 

% .. focusing on students' experiences in complementing (1) conceptual SE learning and (2) software implementations. Additionally, we investigated their overall experiences in using these tools.

%
% Dropping Bloom's and doubling down on engr education paper that draws from Bloom's. 
% With a focus on holistic experiences across lower and higher order cognitive processes in SE learning, 
%With a focus on elicting comprehensive academic experiences of using genAI across SE learning, 


% by asking participants to reference specific artifacts, i.e., open instances of their past genAI use, as per the processes followed by \cite{lau2023ban}, where they reflected on their experiences through tangible artifacts. 
% Here, participants' previous conversation threads with genAI acted as a foundation to support deeper recollection of their experiences. 

%In the first two parts, we examined: (1) students' reasons for using genAI tools ( for example, "" )

% We grounded these conversations by prompting participants to reference specific artifacts or instances of their past genAI use, as per processes followed by \cite{lau2023ban}, where they reflected on their experiences through tangible artifacts. 
% In our case, participants' past conversation threads with genAI served as a supporting bedrock to facilitate deeper recollection of their experiences. 

%facilitated participants in providing a deeper recollection of their experiences, which allowed our insights to be more closely tied to actual user interactions with genAI tools.


% This technique was inspired by the cognitive walkthrough method \cite{mahatody2010state}, commonly used in Human-Computer Interaction (HCI) studies. In this method, participants discuss their experiences when using a tangible artifact.
% In this segment we inquired about the duration of genAI usage among students, aiming to contextualize their experiences and insights within their SE learning journey. Understanding the length of engagement with genAI tools helped us assess the depth of user experience and the evolution of their perceptions over time. Further, the questions on future intentions and the likelihood of students recommending genAI to their peers served as a proxy [] for their overall satisfaction and perceived value of current genAI tools as an educational resource. 

Results RQ1:

%the circumstances (``when'') and methods (``how'') of their genAI usage, along with (``what'') the perceived benefits and challenges (``what''), alongside the contexts (``where'') these perceptions arise.
%In this section, we address RQ1: \textit{What is the landscape of genAI use amongst SE students?}, as introduced in Section ~\ref{sec:intro}. Through semi-structured interviews, we investigated how SE students use genAI to complement both conceptual learning and practical implementations.  We discuss the circumstances (``when'') and methods (``how'')of their genAI usage. Additionally, we detail their perceived benefits and challenges (``what''), alongside the contexts (``where'') these perceptions arise

% \texttt{Verification}: In the absence of formalized ways of verifying genAI generated content, students rely on brute force approaches: (1) cross-referencing with trusted sources like, \textit{``Google or Stack Overflow to check whether the things [genAI] provided are real'' (P4)} and practical testing by \textit{``by running [genAI provided code], seeing if it works'' (P15)}. 

% According to our interviewees, these benefits were perceived only when they already had familiarity with the domain (L2) or were using genAI tools for basic implementations (I1). P10 highlighted issues in using genAI tools for initial learning (L1), stating, \textit{``when I'm using it to learn, I really don't know how accurate [GPT] is the first time, because I don't know what I don't know''}. P7 metaphorically described, \textit{``for complex stuff, there were more potholes than there were roads''} pointing out the challenges when moving beyond basic implementations. 

Results RQ2:

% \begin{figure*}[!ht]
%     \begin{tabular}{cc}
%         \includegraphics[width=0.495\linewidth]{figures/Assocations L1.png} &
%         \unskip\ \vrule\
%         \includegraphics[width=0.495\linewidth]{figures/Associations I2.png} \\
%          (a) & (b)\\
%      \end{tabular}
%      \vspace{-5px}
%     \caption{Figure needs update. Overall sankuy plot and not phase wise are needed.}
%     \vspace{-8px}
%     \label{fig:sankeys}
% \end{figure*}


% \textit{1) \textbf{Gaps for supporting learning}} primarily arise from genAI's \textit{limited support for in-depth understanding of concepts}, \textit{unsuitability for scaffolding learning}, \textit{inadequate higher-order math and logic support}, \textit{lack of visualization support} \footnote{In free versions (e.g., ChatGPT) as of 2024}, and \textit{inadequate explanations}. P10 stated, \textit{``I know people really talk a lot about how it's very beneficial, but I think it is beneficial just to get some sort of summarization point of view, but never has it helped me get an in-depth understanding''}. GenAI tools are currently unsuitable for scaffolding learning: P12 shared, \textit{``ChatGPT does take away from my learning process just because it gives me that immediate answer without me having to find it. I wait before I ask a super big question just so I can think about it before I see a direct answer''}. It also lacks support for higher-order math and logic: \textit{``what [genAI] gives me is incorrect for advanced mathematical concepts that I'm trying to implement in programming'' (P13)}. Lastly, genAI providing inadequate explanations leads to challenges in \textbf{obtaining proper rationales} (C3): \textit{``It was in CS362 class...GPT or Bard didn't provide a specific reason that I felt was good enough or believable on why [a test case] should be written that way'' (P2)}.

% \textit{2) \textbf{Gaps for supporting implementations}} primarily arise from genAI's \textit{poor debugging support}, \textit{inability to orchestrate code}, and being \textit{unsuited for complex implementation tasks}. GenAI often falters in debugging, with P10 noting, \textit{``Generative AI is not very helpful for debugging. It's not really able to debug things so I don't use it for that anymore.''} When it comes to orchestrating multiple codebases or services, genAI's limitations become apparent. Its utility is reduced for more complex problems and \textit{``...things that are not as rudimentary, as it doesn't orchestrate all the things together''}, making it difficult to \textbf{appropriately use its responses} (C5). Overall, genAI's assistance is often inadequate for complex implementation efforts, as highlighted by P9: \textit{``Once tasks start getting more complex, we need to be careful with it, or it can break the code base.''} 

% \textit{3) \textbf{Gaps in genAI capabilities}} include it's \textit{outdated or incomplete knowledge}, \textit{limited working memory}, and \textit{data skeuomorphism}. 
% % P5 shared, \textit{``[genAI] goes really wrong with non-standard problems or less familiar languages[…]I was trying to do some graphics rasterization on PICO 8 that using Lua, and it wasn't really able to match any instruction set or syntax''}. 
% GenAI's limited working memory places hurdles in \textbf{aligning it to human preferences}(C3): \textit{``for bigger projects or building large apps, it's really tough to work with AI with multiple different files, as its memory is limited'' (P4)}. Training data skeuomorphism is reflected in genAI's tendency to replicate solutions and patterns found on the internet, including mistakes or misconceptions. P1 elaborated: \textit{``The biases that exist in a field gets implanted in AI, and therefore some of the things that are not ideal, are grandfathered in and pulled over not because they were the best way or the right way to do it, but because it is the common way''}, indicating how genAI can reinforce outdated practices or perpetuate common errors. These capability gaps present challenges in \textbf{setting accurate expectations} (C1), \textbf{obtaining proper rationales} (C4), and \textbf{effectively using genAI responses} (C5), limiting its applicability in software engineering. \textit{``I struggle with ChatGPT because I can't interact with it the way I can do with my coworkers. I have to break the problem myself first and give it small chunks of context and not the whole thing''}, shared P3. 

% Participants frequently mentioned that they \textit{steered away from genAI} due to ethical considerations \textbf{(C1)}. P10 articulated this concern: \textit{``I don't use it for any implementations because I don't consider it to be something I have written...And I think until the boundaries become clearer on whether it's right to use it or not, I am not comfortable using it for work that I have to claim as my own''}. Engaging in back and forth exchanges \textbf{(C2)}, coupled with difficulties in obtaining clear explanations \textbf{(C4)} and verifying responses \textbf{(C5)}, cultivated \textit{distrust} and reluctance to adopt AI tools: \textit{``I don't trust generative AI for any critical work, it doesn't provide proper justifications; it's more like a predictive text answer that is hard to verify'' (P2)}. P7 added: \textit{``It apologizes when you confront it, but gives you the same answer again and again. It's better to trust yourself and not the tool''}. These experiences reveal a broader skepticism towards genAI, deterring its broader adoption among software engineering students.

% Participants' willingness to adopt generative AI was mainly influenced by challenges in appropriately using genAI responses \textbf{(C5)}. Yet, specific challenges impacting their willingness varied depending on the context of use. For learners (L1), difficulties in effectively communicating needs \textbf{(C2)} and obtaining proper rationales \textbf{(C4)} led to a sense of \textit{distrust}. P8 noted, \textit{``Sometimes, I can't get it to provide a thorough follow-up when I am learning a topic. There have been times when it offered incomplete explanations, and I fell flat on my face trying to build off that. I don't trust it much anymore''}. Conversely, participants' concerns over ethical considerations \textbf{(C1)} when employing genAI discouraged its use in practical implementations: \textit{``...until the boundaries become clearer on whether it's right to use it or not, I am not comfortable using it for work that I have to claim as my own'' (P10)}. 


% \textit{Similarities and differences in associations} 
% Although patterns were consistent, some distinctions emerged in these associations influenced by the context being either learning-focused or implementation-oriented. We briefly discuss these nuances:

% EMBEDDED THIS IN TASK IMPACT
% Firstly, challenges in obtaining proper rationales \textbf{(C4)} and appropriately using genAI responses \textbf{(C5)} had \textbf{\textit{impact on tasks}} in both initial learning (L1) and advanced implementation (I2) phases. However, some associations varied: in the initial learning phase (L1), an unclear understanding of AI's limitations \textbf{(C1)} along with difficulties in framing the right questions \textbf{(C2)}, led to delays in task progress. P8 mentioned, \textit{``I spent at least 30 minutes fixing my prompts and going back and forth to make it work''}. Conversely, in using genAI for implementations, participants reported instances of task abandonment due to difficulties in aligning AI with personal preferences or processes \textbf{(C3)}. P16 shared, \textit{``I went back and forth multiple times explaining ChatGPT about my process. I needed it to help me with modifying a code with a preset style, but it kept on suggesting its own way which was not useful to my project. I gave up trying to fix the code by myself''}.


% Participants' \textbf{\textit{willingness to adopt generative AI}} was mainly influenced by challenges in appropriately using genAI responses \textbf{(C5)}. Yet, specific challenges impacting their willingness varied depending on the context of use. For learners (L1), difficulties in effectively communicating needs \textbf{(C2)} and obtaining proper rationales \textbf{(C4)} led to a sense of distrust. P8 noted, \textit{``Sometimes, I can't get it to provide a thorough follow-up when I am learning a topic. There have been times when it offered incomplete explanations, and I fell flat on my face trying to build off that. I don't trust it much anymore''}. Conversely, participants' concerns over ethical considerations \textbf{(C1)} when employing genAI discouraged its use in practical implementations: \textit{``...until the boundaries become clearer on whether it's right to use it or not, I am not comfortable using it for work that I have to claim as my own'' (P10)}. 


% \subsubsection{Differences} Having explored the associations between students' challenges with genAI and the subsequent impacts, we highlight the nuances in these associations between learning and implementation phases. Although, most patterns were found to be consistent, some distinctions emerged in these associations influenced by the context being either learning-focused or implementation oriented. 

% \texttt{Similarities} across learning and implementation phases include challenges in \textbf{effectively communicating needs or context} (C2) to the AI, which leads to frustration and self-doubt among students. P2 articulated this issue: \textit{``sometimes when I try to prompt what I need, it doesn't feed it in the responses and sometimes it's the opposite. Those instances are very irritating for me. I feel I am at fault for not asking the smart questions''}. Difficulties in \textbf{obtaining proper rationales} (C4) impact tasks by leaving students to independently navigate or solve problems: \textit{``It outputted sensible looking code but it didn't provide a good explanation, rather it threw me in logic loops. Ultimately, I ended up writing the code from scratch'' (P5)}. Further, the challenge of \textbf{appropriately using genAI responses} (C5) affects tasks, tool adoption, and leads to frustration. P4 reflected: \textit{``If I am frustrated with it when it does not help, I don't go back to prompt it more because it has been a longer waste of time. I would fall back, and look at other solutions, or ask other people to help me [...] and shift to the pre-AI era learning style when AI wasn't a thing.''} 

% \texttt{Differences} are influenced by whether students engage with genAI tools for learning purposes or practical implementations. For learning, the \textbf{impact on tasks} stem from an \textbf{unclear understanding of AI's limitations} (C1) and challenges in \textbf{framing the right questions or providing sufficient context} (C2), which tend to slow down students' progress: \textit{``I spent at least 30 minutes fixing my prompts and going back and forth to make it work'' (P8)}. Conversely, during implementation phases, the difficulty in \textbf{aligning AI with individual preferences or processes} (C3) often lead to frustration and abandonment of tasks.

% \textbf{Tool adoption} is similarly affected by varied challenges. In learning scenarios, \textbf{lack of proper rationales} (C4) and the \textbf{need for domain knowledge to query AI effectively} (C2) steer students away from using these tools. In contrast, during implementation, difficulties in \textbf{using AI responses effectively or verifying them} (C5) fosters distrust towards genAI.

% The challenge of \textbf{aligning AI with individual processes or preferences} (C3) also has nuanced impacts. For learners, difficulties in matching genAI's approach to their learning styles lead to an incomplete understanding of concepts, significantly affecting the learning outcome: \textit{``I am not able to use AI [...] in the way I like to learn'' ( P1)}. Conversely, in implementation tasks, the \textbf{inability to adapt AI responses to meet specific requirements} (C5) slows down progress or causes students to completely abandon the task at hand. Notably, the issue of \textbf{unclear genAI limitations} (C1) is particularly problematic for beginners in the learning phase (L1), who might over-rely on genAI, trusting its responses blindly: \textit{``when I trusted it too much, and built off the information it provided, I fell flat on my face. It didn't actually do things the right way'' (P3)}.





% Inconsistent and incorrect responses were common, with P15 noting, \textit{``Sometimes ChatGPT would just say things that were plainly incorrect"}. GenAI also provides incompatible responses, as highlighted by P2: \textit{``I was asking about a specific software design, and essentially it gave me good information, but it wasn't for the correct label and I couldn't use it”}. P1 expressed difficulties due to incomplete assistance: \textit{"There will be times where it's very sparse and very difficult to get the quality of answer that I'm looking for out of it"}. Additionally, P3 described the challenge of receiving suboptimal solutions: \textit{``It doesn’t actually do things the right way...basically I was learning unoptimal ways of writing code, and doing software development''}. P15 pointed out genAI's limited specificity issue: \textit{``It's the specifics for which ChatGPT breaks down[...]it gets choked up on the specifics''}. P3 illustrated difficulty in generalizing genAI solutions: \textit{``sometimes it would give me solution to a prompt, very specific to that one instance and its responses would be very hard to generalize or modify to include all cases''}.

Discussion: 

% Instructors aiming to incorporate genAI into their curricula should be aware of the difficulties that students might encounter when using genAI for initial learning (L1) and advanced implementations (I2). A significant obstacle in adopting this rapidly developing technology is understanding its limitations and applicability. Relying too heavily on genAI [] is particularly harmful to learners, as they may accept the AI's output as definitive, rather than taking responsibility for their own work. Hence, instructors must educate students about the workings of genAI and its faults, emphasizing the need for verification of its outputs, given that these systems are language, not knowledge models; generating plausible word sequences without guaranteeing the veracity of the information. Setting clear expectations regarding genAI's assistance can help students, especially beginners (L1), to scope their trust in AI [...] and use it effectively, instead of treating it like an expert. Further, rather than penalizing students for using genAI, which will only lead to more creative ways of academic misconduct, students should be guided on ethical practices and the importance of acknowledging AI’s role in their work. 

%Use GenAI as part of the tool belt, but explore the landscape first. Students must be educated to use genAI as a resource and explore the possibility of different prompts keeping in mind that it may require a basic understanding of the SE concepts and the goal they have in mind before prompting. Moreover, it is important to be critical of the output received and seek to understand the details by asking more specific questions or triangulating with other reliable sources. 


%create tutoring systems tailored to the learner's background, conversational patterns, and help-seeking intentions. This approach aims to create more personalized teaching strategies, moving away from a generic one-size-fits-all approach. By evolving these tools into adaptive conversational agents, there is an opportunity to improve students' problem-solving abilities and meta-cognition skills.

% Threats
%\textbf{\textit{Construct validity}} involves ensuring the accuracy of constructs, potentially compromised by asking incorrect questions. To minimize this threat, we assessed the interview script's validity through sandboxing and pilot sessions until a team consensus was reached. Another threat could arise from the absence of concrete tasks during the study, limiting our results to our participants' recollections. We reduced this by focusing discussions on concrete artifacts to elicit participant experiences. Despite these measures, we recognize the potential for measurement inaccuracies.

\iffalse

% Where to use section (see intro boldification section before coming here):

% ** Need for educating students, educators, policy makers of where genAI is helpful and insights for AI designers for things to improve to expand the “it depends” spectrum. 

% % Food for thought:
% % Connection to bloom
% % Aligning to process/preference effecting learning and implementations - GenderMag
% % Where to use/not use? Recommendations for educators, recommendations for AI designers???

% % Maybe's:
% % Perspectives and future use
% % Anthropomorphism

The new landscape:
- Basics of how to use....strategies

- instructors: calculator --> 

** genAI should be used for incremental learning and basic implementations. 

** Doesn’t take away from learning, rather complements it – as students using it to refine knowledge have some capacity to judge the “truthfulness” and using it for basic implementations fastracks blockers by providing help (boilerplates, examples) for the repetitive and "boring" tasks.

---------

Students + Instructors: When [stage of learning] and How [different strategies that we identified] students can use genAI (direct from results??) need formal learning before using it. 

Students: How to use, what to expect [Be aware of the faults...and how to safeguard from these]

Instructors: what kind of assignment, how to include AI stuff in their education

What kinds of information would the students need when using genAI (how to help with the literacy) need to know about AI


Implementation: good starting point not ending point. Owing the soln is what students need to do. You are responsible for the final part...cant blame AI and be careful of ethics - You need to own it... Trust but verify.

Recommendations:

- for initial learners
- trust and verify



Recommendations for SE educators/ Considerations for adoption:
  where to use + calculator example - highlighting how AI can be used to kickstart things. how to? trust but verify.
  where to not use - initial learning and advanced implementations. Why's? initial - learn wrong, not asking right questions, not being able to verify, hit on cognitive skills (+ Aligning is a problem, AI doesnot behave the way humans do)

Recommendations for AI designers:
tools are "stubbornly opaque"
  Scaffold learning













----------------------------------OLD----------------
** Educator Guidelines for AI in Education (Where/What)

** Drawing a parallel to the calculator era too.

** genAI should be used for incremental learning and basic implementations. 

** Doesn’t take away from learning, rather complements it – as students using it to refine knowledge have some capacity to judge the “truthfulness” and using it for basic implementations fastracks blockers by providing help (boilerplates, examples) for the repetitive and "boring" tasks.

** AI people
% - anthropomorphism: the way AI talks can influence over(reliance). 
- match cognitive style: Our findings show that not aligning to users style lead to impacts on learning and on task. Transit to cognitive tax and then to GMag of how it can be used by AI designers. They should tailor AI responses based on understanding the users cognitive style. GMag to the rescue. 

** Researchers: Calculator vs LLMs
- Reflection/Problem solving -> Code comprehension

What kind of probl;em solving goes away
What can it impact
How should LLMs be especially for students /scaffold reflection and problem solving by students "answer garden" - Peggy work. 


Implications for ICSE matching:

Papers that focus on human, social, economic and socio-technical aspects without a direct impact on software engineering, development, research and/or education 
Papers that innovate or study the design of software from the perspective of end users that are not software engineering stakeholders (e.g., website design) 
Papers that report on human and social theories that do not consider the context of software engineering development, software research and software education (e.g., a theory of how a mobile app can drive behaviour change)





Ai is everywhere and SE students needs to know before they get out. We find where and how they are using it and findings will help in fig guidelines. 


\fi

==> sec/old-method.tex <==
% Participants from highlighted: https://docs.google.com/spreadsheets/d/1BmtU8RFdWvCpdPpPXJcdcXQB6S-VtIyN/edit#gid=115791237

% \section{Method}
% \label{sec:method}
% We answered our RQs by conducting semi-structured interviews with students who have used genAI to complement their learning and implementations while taking software engineering courses. Following best practices in qualitative research \cite{creswell2016qualitative}, we did not segregate the interviews and data analysis into distinct phases, instead, we continuously refined our understanding, making adjustments to our interview script and code set throughout the interviews.
 
% % Please fix as you see fit. The comments will get cluttered up soon. 
% \subsection{Interview Planning}
% \subsubsection{Interview Script}
% % What is blooms. Can be divided into lower and higher.
% We aligned our exploration with an educational framework, such as Bloom's taxonomy [], to allow a holistic examination of student experiences with genAI for complementing SE learning. This taxonomy categorizes learning objectives across a continuum of cognitive processes: from \textit{lower order processes} involving acquisition and understanding of knowledge (remembering, understanding), to \textit{higher order processes} that promote application and synthesis of knowledge into new contexts (applying, analyzing, evaluating, and creating). 

% Given our focus on different levels of Bloom's Taxonomy, we structured our interviews \footnote{Refer to supplemental for interview script: [link]} into 3 parts: (1) Experiences in learning concepts with genAI, addressing \textit{lower order processes}; (2) Experiences in implementing solutions with genAI, focusing on \textit{higher order processes}, and (3) Overall experiences with genAI.


% \textit{Experiences in Learning}: The first segment of the script focused on students' experiences with genAI for learning software engineering. This segment was anchored in Bloom's lower-order cognitive processes. To capture student experiences, we explored: 
% (1) What motivated them to use genAI to complement their SE learning? (2) What challenges did they face in their learning with genAI? and (3) When they faced challenges, how did they surmount them?

% This helped us identify the issues in the educational context, including AI gaps, faults, or limitations in the technology itself. 

% By probing into how students dealt with these challenges we gained insights into their adaptive strategies to navigate the challenges, technological faults, and limitations.


% \textit{Experiences in Implementing Solutions}: The second segment of our script explored Bloom's higher-order cognitive processes by investigating the use of genAI for SE implementations in projects and exercises. Aligned with the first part, we sought to understand (1) students' motivations behind using genAI, (2) the challenges encountered in the process, and (3) the employed strategies to surmount the challenges.

==> table/course-content-old.tex <==



\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|p{0.11\textwidth}|p{0.2\textwidth}|p{0.2\textwidth}|}
\hline
\textbf{Category} & \textbf{CS361} & \textbf{Capstone} \\
\hline
L1 (Initial Learning) & 
\begin{itemize}[nosep,leftmargin=*]
\item Basic concepts (Git, APIs, UI)
\item Software process models
\item Intro to testing concepts
\end{itemize} & 
\begin{itemize}[nosep,leftmargin=*]
\item Project requirement analysis
\item Architectural patterns
\item Documentation best practices
\end{itemize} \\
\hline
L2 (Incremental Learning) & 
\begin{itemize}[nosep,leftmargin=*]
\item Advanced Git features
\item RESTful services design
\item Compare process models
\item Detailed Scrum practices
\end{itemize} & 
\begin{itemize}[nosep,leftmargin=*]
\item API gateway design
\item Performance monitoring
\item OAuth security
\item Advanced testing techniques
\end{itemize} \\
\hline
I1 (Initial Implementation) & 
\begin{itemize}[nosep,leftmargin=*]
\item Framework setup
\item Basic UI creation
\item Third-party API integration
\item Simple unit testing
\end{itemize} & 
\begin{itemize}[nosep,leftmargin=*]
\item Multi-service environment config
\item Prototype building
\item Automated testing setup
\end{itemize} \\
\hline
I2 (Advanced Implementation) & 
\begin{itemize}[nosep,leftmargin=*]
\item Complete project building
\item Code review practices
\end{itemize} & 
\begin{itemize}[nosep,leftmargin=*]
\item Cloud deployment (Github pages, AWS)
\item Integrate your code with other microservices
\item CI/CD implementation
\item Maintenance routines
\end{itemize} \\
\hline
\end{tabular}
\caption{GenAI Usage in CS361 and Capstone Courses}
\label{tab:course-content-old}
\end{table}
